Powering the Next Billion Devices with Wi-Fi

We present the first power over Wi-Fi system that delivers power and works with existing Wi-Fi chipsets. Specifically, we show that a ubiquitous piece of wireless communication infrastructure, the Wi-Fi router, can provide far field wireless power without compromising the network's communication performance. Building on our design we prototype, for the first time, battery-free temperature and camera sensors that are powered using Wi-Fi chipsets with ranges of 20 and 17 feet respectively. We also demonstrate the ability to wirelessly recharge nickel-metal hydride and lithium-ion coin-cell batteries at distances of up to 28 feet. Finally, we deploy our system in six homes in a metropolitan area and show that our design can successfully deliver power via Wi-Fi in real-world network conditions.

==> battery-1.tex <==
\subsection{Battery-charging Efficiency}
XXX



==> benchmarks.tex <==
\section{Benchmark Results}\label{sec:benchmarks}

As described in \secref{sec:design}, \name is designed to provide high channel
occupancy to deliver power while having a minimal effect on Wi-Fi traffic. In
this section, we evaluate this property in more detail. Specifically, we deploy
\name on a Wi-Fi router and configure it to transmit using the mechanisms
designed in \xref{sec:design} on Wi-Fi channels 1, 6, and 11.

We tested \name in multiple benchmark scenarios to evaluate its effect on client
traffic.  In our experiments, a single desktop PC with three Atheros AR9580
802.11g cards acts as the access point (AP), and Dell Inspiron 1525 laptop
clients using identical Atheros cards connect to the Internet via NAT on the AP.
%
The four main scenarios are:
\begin{itemize}
\item \term{Baseline}: \name is disabled on the AP; the AP introduces no extra
traffic.  In this case, an RF-harvesting device can harvest only when the AP is
transmitting normal client traffic or short Wi-Fi beacons.
\item \term{Blind UDP}: \name is disabled, but a userspace program on the AP
emits broadcast UDP traffic on all of its wireless interfaces.
\item \term{\name}: the AP broadcasts \name traffic (UDP broadcast with the
\name IP option set) at the interface's maximum bitrate.
\item \term{\name-slow}: the AP broadcasts \name traffic at a slower bitrate to
take more time on the channel with each frame.
\end{itemize}

We evaluate \name with four different Wi-Fi traffic patterns and metrics:
%
1) the page load time (PLT) of the ten most popular websites in the United
States~\cite{alexa-topsites},
%
2) the throughput and jitter (XXX no jitter data) of UDP download traffic at
various bitrates, and
%
3) TCP download throughput as a function of different Wi-Fi bit rates.
%
We finally evaluate the effect of \name on other Wi-Fi networks in the vicinity
of our benchmarking network.

\textbf{Measuring channel occupancy.}
The occupancy of a channel, measured in percent, is a key metric in WiFi
networks because it influences how often stations using carrier sense will
be able to transmit.
%
\secref{sec:design} describes our rationale behind measuring occupancy using
frame metadata at the AP.
%
We use a simple technique to compute \name's contribution to channel occupancy.
First, we use \lil{aircrack-ng}'s \lil{airmon-ng} tool to add a monitor
interface to the interface serving AP traffic (e.g., \lil{mon0} refers to the
same interface as \lil{wlan0}).  We then start \lil{tcpdump} on the monitor
interface to record all traffic including radiotap headers (802.11 frame
information, including retransmissions).  Finally, we stop \lil{tcpdump} and use
\lil{tshark} to extract frames sent by the AP, recording the bitrate and
frame size for each frame.  The average channel occupancy for the capture file's
recording period is therefore
\begin{equation}
100\% \times \left(\sum_{i\in \mathit{frames}}
(\mathit{framelen}_i \times 8) / \mathit{rate}\right) / \mathit{duration}.
\label{eq:occupancy}
\end{equation}

This method of occupancy more closely approximates the Wi-Fi card's contribution
to traffic on the channel than two other approaches we tried: reading hardware
channel survey information, and using information from a software-defined radio
(SDR) such as GNU Radio.  SDR is unwieldy and is not built into routers, which
is a key feature of \name. XXX say more.

XXX note that other nodes on the same channel can affect these channel occupancy
measurements, since our measurement captures only the AP's own traffic.  Since
the AP obeys the MAC protocol, other traffic on the channel will reduce the AP's
share of the channel's traffic.

\vskip 0.05in\noindent{\it (a) Page load time.}
To evaluate the effect of \name on bursty, unpredictable client traffic, we
place the Wi-Fi client 2 meters from the Wi-Fi router and measure how quickly
popular webpages load.  A test harness uses the PhantomJS headless
browser~\cite{phantomjs} to download the front page of each of the ten most popular
websites in the United States (ranked by Alexa~\cite{alexa-topsites}) 100
times, clearing the cache and pausing for one second in between page loads.  We
record the page-loading traffic with \lil{tcpdump} and analyze it offline to
determine page load time and average channel occupancy (\qref{eq:occupancy})
over the 100 trials.

The Wi-Fi devices use the standard Atheros/hostapd rate adaptation to modify
their rates.  The experiments were performed in a busy office environment where
there were tens of other clients and routers on all 2.4~GHz Wi-Fi channels.

\begin{figure*}[t]
\centering
\includegraphics[width=0.32\textwidth]{pageload_results/plt-baseline}
\includegraphics[width=0.32\textwidth]{pageload_results/plt-noipopt}
\includegraphics[width=0.32\textwidth]{pageload_results/plt-power}
\caption{For the page load time experiment, \name's average effect on page load
time for a client was only $X\%$ (middle figure), versus $Y\%$ when blindly
broadcasting UDP traffic (rightmost figure).
\textbf{XXX} replace with an ASPLOS-ish speedup/slowdown figure with results
normalized to baseline.}
\label{fig:plt-performance}
\end{figure*}

\figref{fig:plt-performance} shows the average PLTs for each of the websites
both with and without \name, and with blind broadcast UDP traffic that does not
obey \name's queue-depth threshold rule. The figure shows the following:
\begin{itemize}
\item Blind broadcast UDP traffic results in a $Y\%$ average slowdown versus
the baseline for the ten websites.
\item \name causes less performance degradation ($X\%$ average slowdown) than
blind broadcast UDP, illustrating the benefit of \name's queue-depth
threshold rule.
\item To further understand the results, in plot the CDF of page load times for
amazon.com for the 100 trails with and without \name. The figure shows that
XXX.
\end{itemize}

\begin{figure*}[t]
\centering
\includegraphics{pageload_results/plt-occupancy}
\caption{For the page load time experiment, the sum of the per-channel
occupancies remains high regardless of the webpage being loaded.}
\label{fig:plt-occupancy}
\end{figure*}

\figref{fig:plt-occupancy} plots the channel occupancies as observed in each of
the three channels (1, 6, and 11) for the \name and blind UDP scenarios.  Since
the sum of the channel occupancies across Wi-Fi channels is the \emph{effective}
channel occupancy a harvester observes, \name's goal is to increase its
\emph{total} occupancy across all channels.  The figure shows that the total
channel occupancy is generally above 80\%, high enough to provide sufficient
charge to harvesters in our tests.

\vskip 0.05in\noindent{\it (b) UDP Download traffic.}
Next, we evaluate \name's effect on \emph{streaming} traffic over a UDP
connection.  This is a common scenario for many media applications such as video
streaming.
We reproduce the experiment setup in the page load experiments, but now we
run iperf on the client and AP.  The client is at a fixed distance of
$2\,\text{m}$.  The client sets a target Wi-Fi bitrate (e.g., $54\,\text{Mbps}$)
and runs five sequential copies of iperf, 3 seconds apart.
iperf measures throughput over  $500\,\text{ms}$ intervals. We repeat the
experiments with target UDP bitrates of 1, 5, 10, 15, 20, 25, 30, 35, 40, 45,
and 50 Mbps, and measure the achieved bitrate over all trials in the scenarios
described above.

\figref{fig:udp-throughput} plots the average UDP throughput achieved both with
and without \name as a function of the eleven tested UDP data rates.  The figure
shows that the client's iperf traffic achieves roughly the same rate with \name
as it does without any power traffic (the baseline).
%
This result demonstrates that \name effectively prioritizes client traffic above
power traffic as the target bitrate increases.  With blind UDP broadcast
traffic (the ``noipopt'' scenario in the figure), the AP's kernel does not
prioritize the client's iperf traffic over the power traffic, resulting in
roughly a halving of the iperf traffic's bitrate as the AP shares the channel
fairly.

\begin{figure*}
\centering
\includegraphics{udp_iperf_results/udp-iperf}
\caption{UDP throughput.}
\label{fig:udp-throughput}
\end{figure*}

\figref{fig:udp-occupancy} plots channel occupancy as a function of UDP data
rate. The figure again plots the occupancies on all channels with and without
\name as well as the cumulative channel occupancy across all the Wi-Fi channels.
The plot shows that \name's cumulative occupancy is generally above 80\% as in
the PLT experiment.

XXX we did not measure jitter.  To understand how \name affects the packet
delays, we plot the CDF of the inter-packet arrival time both with and without
\name. We plot  the delay results for the UDP data rate of XXX~Mbps. The figure
shows that XXX.

\begin{figure*}
\centering
\includegraphics{udp_iperf_results/udp_cdf}
\caption{UDP occupancy.}
\label{fig:udp-occupancy}
\end{figure*}

\vskip 0.05in\noindent{\it (c) TCP Download traffic.} We repeat the previous experiments with iperf but now with TCP. Specificallt, we run iperf on the client for a duration of XXX minutes and compute the throughput achieved at the client over durations of 500~ms. We repeat the experiment for various Wi-Fi bit rates. Specifically, we run the experiments for XXX different Wi-Fi bit rates of XXX, XXX and XXX Mbps. The client is placed XXX meters away from the router.

\begin{figure*}
\centering
\includegraphics{tcp_iperf_results/tcp_tput_cdf}
\caption{TCP throughput.}
\label{fig:tcp-throughput}
\end{figure*}

\figref{fig:tcp-throughput} plots the average TCP throughput achieved both with and without \name as a function of the WI-Fi data rates. The plots show that XXX. 

To understand how \name affects the packet delays, we plot the CDF of the inter-packet arrival time both with and without \name. We plot  the delay results for the Wi-Fi bit rate of XXX~Mbps. The figure shows that XXX.


As before, we also plot the channel occupancies values as a function of the
Wi-Fi data rates (\figref{fig:tcp-occupancy}). The plots show that XXX.

\begin{figure*}
\centering
\includegraphics{tcp_iperf_results/tcp_cdf}
\caption{TCP occupancy.}
\label{fig:tcp-occupancy}
\end{figure*}

\vskip 0.05in\noindent{\it (d) Effect of other Wi-Fi network traffic.} The algorithm in~\xref{blah} ensures that the power packets transmitted by \name have a minimal effect on the other transmissions at the Wi-Fi router and are fair with other wi-Fi networks in the environment. Specifically, it uses the inherent fairness of the Wi-Fi MAC to ensure that \name is fair to other Wi-Fi network. To evaluate this, we run experiments in the presence of another Wi-Fi network. Specifically, we place our Wi-Fi router in the vicinity of our organization's Wi-Fi network. We configure our Wi-Fi router to transmit packets using our algorithm on channel 1 and channel 2. We place a client that is associated with our organization's network on Channel 1 and we run iperf with UDP traffic on the client with varying UDP data rates. We run the iperf for a duration of XXX [explain in detail how the throughput values are computed].

Figure~\ref{blah} shows the throughput for both the UDP throughput on the client as well the rate of the power packets transmitted on Channel 1. The figure shows that XXX..   




\section{Evaluating the Harvesting Hardware}
We design our harvester circuit to be efficient across all the 2.4~GHz Wi-Fi channels and have good harvesting efficiencies. 
The sensitivity and the efficiency of an RF energy harvesting front end is a function of input power, leakage of the platform and the desired output voltage. Hence, it is imperative that we evaluate the harvester at a system-level that takes into account all these factors. In this section, we evaluate our hardware versus these  parameters that effect its performance.


\vskip 0.05in\noindent{\it (a) Matching efficiency versus frequency.} Efficiency/matching across frequency is measured using return loss (RL) which is the amount of power which is reflected (lost) at the antenna interface. This occurs because XXX (explain this in more details). The matching network used in our design in~\xref{blah} is to minimize these reflections/loss while remaining efficient across multiple 2.4~GHz Wi-Fi channels. We return the return loss by XXX (explain in detail how you are running the experiments). 

Fig.~\ref{blah} plots the XXX. It shows that XXX.


\vskip 0.05in\noindent{\it (b) Understanding the power-conversion efficiency.} The power-conversion efficiency is defined as the fraction of received RF power at the input of the energy-harvesting circuit that is converted into useful power that can power the microcontroller and the sensors. These efficiencies numbers are typically low due to the inherent nonlinearities of diodes that reflect some power when the circuit is not completely matched. Further, due to the diode non-linear effects, the efficiency numbers are a non-linear function of the input RF power. To understand the power-conversion efficiencies of our harvesting design, we do XXX (explain the experiment).

Figs.~\ref{blah} (a) and (b) shows these efficiencies values as a function of the input power. The results are plotted by for our battery-free harvesting hardware (Fig.~\ref{blah}(a)) as well as a battery-rechargable harvesting hardware (Fig.~\ref{blah}(b)). We plot the results at transmissions in various Wi-Fi channels. The plots show the following:
\begin{itemize}
\item XXX
\item XXX
\end{itemize}


==> details.tex <==
\section{XXX Uncategorized Details}

To measure the effect of \name on \emph{bursty} client traffic, we measured
webpage loading time with and without \name.
%
We used the headless browser PhantomJS~\cite{phantomjs} to repeatedly load the
front pages of the top 10 websites in the United States as ranked by
Alexa~\cite{alexa-topsites}.

Implementation note on broadcast traffic on Linux: note that we had to connect
clients to each of the AP's channels before the AP would actually send UDP
broadcast packets/frames on those channels.

\textbf{You have just re-invented QoS.  Why not just use traffic shaping?}
We adopt the concept of traffic shaping from previous work on enforcing
quality-of-service guarantees.  However, we elected not to use the existing QoS
tools such as Linux queuing disciplines and traffic control (\texttt{tc})
because they operate at the IP layer, whereas \name uses information from the
MAC layer to inform IP-layer queuing decisions.


==> fcc.tex <==
\section{FCC Rules}

Clearly the easiest and most naive way to power devices using Wi-Fi is to blast as much power as technically possible.
However, governments around the world have placed limits on EM emmissions to protect public safety and reduce interference.
In this section, we will explore the implications of the U.S. Federal Communication Commision's EM emissions limits on Wi-Fi power harvesting.

% What about field strength? fundamental: 50 uV/m, harmonics: 500 uV/m

Wi-Fi devices are classified as digitally modulated intentional radiators operating in the 2400-2483.5 MHz (ISM) band. % what about 5 GHz?
In this band, the output power of a device must not exceed 1 W (30 dBm).
Additionally, for each dB of directional antenna gain above 6 dBi, the transmitter must reduce it's output power by the same amount in dB.~\cite{fcc-47.15.247}
Thus, the maximum conducted output power allowed can be simply calculated by:

\[
P_{max} =  \left\{
  \begin{array}{l l}
    30 \text{\ dBm}           & \text{if\ } G_{ant} \le 6 \text{\ dBi}\\
    36 \text{\ dBm} - G_{ant} & \text{if\ } G_{ant} > 6 \text{\ dBi}\\
  \end{array}\right.
\]

\noindent where $P_{max}$ is the maximum allowed output power and $G_{ant}$ is the gain of the antenna.

These rules, however, contain some ambiguity, particularly relevant when trying to power devices.
Namely, what is meant by ``output power'' and what happens when we have multiple antennas?

% Output Power
When calculating ``output power'' to determine compliance with current FCC regulations there are two options: maximum peak conducted output power and maximum conducted output power.
Maximum \textit{peak} conducted output power is measured using a peak detector and limits the \textit{peaks} of the transmitted signal to the $P_{max}$ discussed above.
Measuring maximum conducted output power is allowed as an alternative to maximum peak conducted output power and is generally measured by averaging the power over a bandwidth of 1 MHz for the entire emmission bandwidth and summing the spectral levels.~\cite{fcc-measure-guidance} % over all symbols, can't be during a time of low power transmission, etc.
For harvesting Wi-Fi signals, this second method tends to be better due to its tolerance of higher peak to average power ratios.

% Multiple Antennas
Given these definitions of output power, the rules are fairly straightforward for devices with a single antenna.
However, many Wi-Fi devices include multiple antennas and this leaves the question: how do you calculate ``directional antenna gain'' for multi-antenna systems?

It turns out that the way to calculate ``directional antenna gain'' for multi-antenna systems depends on the type of transmission.
The FCC classifies digital transmissions into two categories: correlated and uncorrelated.
Correlated signals, beamforming being a notable example, have the potential of increasing the field strength at a particular location above that for a single antenna device.
When transmitting correlated signals, the directional antenna gain is calculated by

\[
G_{dir} = G_{ant} + 10 \text{ log}_{10}(N_{ant}) \text{ dBi}
\]

\noindent where $G_{dir}$ is the directional antenna gain for use in Equation ?, $G_{ant}$ is the antenna gain of the individual antennas (assumed to all be the same), and $N_{ant}$ is the number of antennas.

Alternatively, if the transmit signals are completely uncorrelated, spatial multiplexing for example, the directional antenna gain is calculated by

\[
G_{dir} = G_{ant}
\]

\noindent and no adjustments are needed to take into account multiple antennas.
In all cases, maximum conducted output power is summed accross all antennas (in linear units). ~\cite{fcc-multiple-transmitter-output}

Since there is a required backoff of a dB for each antenna when using beamforming while spatial multiplexing has no backoff, this indicates that there will be no power harvesting benefit to beamforming compared to spatial multiplexing.
In fact, since beamforming is never perfect and a 3 antenna system cannot completely regain the required 3 dB backoff in beamforming gain, a beamforming solution will be strictly worse than a solution that uses uncorrelated signals.
We explore this topic more in later sections.



==> fitbit-1.tex <==
\section{Wi-Fi as a Charging Hotspot}
\label{sec:fitbit}

\begin{figure}[t!]
\vskip -0.1in
\centering
{\footnotesize
\begin{tabular}{c}
\includegraphics[width= 0.6\columnwidth]{./figures/images/usb_charger.png}
\end{tabular}
}
\vskip -0.15in

\caption{The FitBit charging prototype which harvests Wi-Fi signals to charge a FitBit device. The prototype consists of a rectifier followed by the standard USB charging cable of a FitBit device. \textnormal{Place holder, replace with a nicer picture}}

\label{fig:cw_wifi_rectifier}
\vskip -0.09in
\end{figure}

In addition to powering custom temperature and camera sensors, we also demonstrate that Wi-Fi routers can be repurposed to serve as wireless charging hotspots for wearables such as a FitBit Flex device~\cite{fitbitflex}. Ideally, a clean-slate design would repurpose the Fitbit's 2.4~GHz Bluetooth antenna and replace its battery charger with our custom battery charger hardware. However since we do not have access to the FitBit's internals, we develop a custom charging solution in Fig.~\ref{fig:cw_wifi_rectifier} that harvests Wi-Fi signals to recharge the FitBit's internal battery. Specifically, we use a 2~dBi 2.4~GHz antenna attached to our harvesting rectifier board, which in turn plugs into the standard USB charging cable.


We place a \name\ router on a table and leave four FitBit Flex devices that have been discharged (i.e., battery has no charge) in the vicinity of the router. All the FitBits are placed  10--15~cm from the router. The router runs the algorithm in~\xref{blah} on the three 2.4~GHz Wi-Fi channels. We leave the setup running overnight and compute the time it takes to fully charge the devices. [XXX:explain how you note full-charge]. As a baseline, it takes a plugged-in FitBit Flex XXX  hours to fully charge from a no-charge state. Fig.~\ref{blah} shows the wireless charge time for the four devices. The average charge time is XXX hours, and all the devices were fully charged over the course of a night. This demonstrates the feasibility of turning a Wi-Fi router into a hotspot near which devices can be left to recharge. We also note that near-field charging solutions require spiral coils to be placed inside the device. Wearables such as FitBits are severely size constrained, which indirectly limits the coil size. Since the operating range of near-field systems is directly proportional to the coil size~\cite{XXX,XXX}, the range of near-field solutions is more limited than the 10--15~cm achieved by \name. In contrast, one can, in principle, repurpose existing 2.4~GHz antennas on wearable devices to harvest power from Wi-Fi and charge multiple devices in the vicinity of the router.


==> futurework.tex <==
Adaptive power duty cycling with feedback loop from device being powered.

